Mix3D: Out-of-Context Data Augmentation for 3D Scenes

We present Mix3D, a data augmentation technique for segmenting large-scale 3D scenes. Since scene context helps reasoning about object semantics, current works focus on models with large capacity and receptive fields that can fully capture the global context of an input 3D scene. However, strong contextual priors can have detrimental implications like mistaking a pedestrian crossing the street for a car. In this work, we focus on the importance of balancing global scene context and local geometry, with the goal of generalizing beyond the contextual priors in the training set. In particular, we propose a "mixing" technique which creates new training samples by combining two augmented scenes. By doing so, object instances are implicitly placed into novel out-of-context environments and therefore making it harder for models to rely on scene context alone, and instead infer semantics from local structure as well. We perform detailed analysis to understand the importance of global context, local structures and the effect of mixing scenes. In experiments, we show that models trained with Mix3D profit from a significant performance boost on indoor (ScanNet, S3DIS) and outdoor datasets (SemanticKITTI). Mix3D can be trivially used with any existing method, e.g., trained with Mix3D, MinkowskiNet outperforms all prior state-of-the-art methods by a significant margin on the ScanNet test benchmark 78.1 mIoU. Code is available at: https://nekrasov.dev/mix3d/

==> 3dv_tables/exp1_context_during_training.tex <==
% !TEX root = ../3dv_mix3d_paper.tex

\begin{table}[h]
    \centering
    \begin{tabular}{l c c  }
        \toprule
        Method & Crop-size & mIoU \\
        \midrule
        \multirow{5}{*}{KPConv~\cite{thomas19ICCV}} 
               & $0.5$ & $53.8$ \\
               & $1.0$ & $67.2$ \\
               & $1.5$ & $68.5$ \\
               & $2.0$ & $69.3$ \\
               & $3.0$ & $69.6$ \\
               \cline{2-3}
               &\namelong{} & $\mathbf{70.4}$\\
        \midrule
        
        \multirow{3}{*}{MinkowskiNet~\cite{Choy2019CVPR}} &
        1/16-scene & 65.4 \\
        &1/4-scene & 66.9 \\
               & full scene & 66.6  \\
               \cline{2-3}
               &\namelong{} & \textbf{69.0}\\
        \bottomrule
    \end{tabular}
\caption{
\small \textbf{Influence of crop size.}
We train KPConv and MinkowskiNet on crops of input scenes, \ie the input to KPConv are spheres with an increasing radius and for MinkowskiNet, the input scene is divided into $n$ chunks which are individually fed to the model.
    We observe that the regularization effect of context invariance cannot be achieved by simply training on cropped regions, as \namelong{} outperforms all tested cropping configurations.
    We report a significant performance gap of $+2.4\%$ when trained with maximal crop sizes on MinkowskiNet, \ie full scenes.
    For KPConv, \namelong{} is applied with $2$m crops and for MinkowskiNet we use full scenes.
}
\vspace{0pt}
\label{tab:cropping}
\end{table}


==> 3dv_tables/exp5_comparison_sota_per_class.tex <==
% !TEX root = ../3dv_mix3d_paper.tex

\begin{table*}[t]
\begin{center}
\begin{tabular}{rcc|ccccccccccccc}
\toprule
Method	 & \namelong{} & mIoU & ceiling	 & floor	 & wall	 & beam	 & column	 & window & door	 & chair	 & table	 & bookshelf	 & sofa	 & board & clutter \\
\midrule
MinkNet\,\cite{Choy2019CVPR} & \xmark & 64.8 & 92.6 & 96.4 & 82.0 & 0.2 & \textbf{28.1} & 53.3 & 64.1 & 87.7 & 78.5 & \textbf{73.8} & 65.5 & 63.1 & 56.4 \\
(5cm)& \cmark & \textbf{65.5} & \textbf{93.5} & \textbf{97.5} & \textbf{82.8} & 0.0 & 24.3 & \textbf{57.5} & \textbf{64.8} & \textbf{88.6} & \textbf{80.7} & 72.9 & \textbf{62.6} & \textbf{68.3} & \textbf{57.5} \\
\midrule
KPConv\,\cite{thomas19ICCV} & \xmark & 65.0 & 93.6 & 98.3 & 81.9 & 0.0 & \textbf{19.4} & 54.8 & 64.7 & 91.1 & 81.4 & 74.4 & 64.2 & 63.0 & 58.0 \\
(Rigid)& \cmark & \textbf{66.5} & \textbf{93.9} & \textbf{98.4} & \textbf{82.9} & 0.0 & \textbf{19.4} & \textbf{59.4} & \textbf{69.0} & \textbf{91.3} & \textbf{81.6} & \textbf{75.6} & \textbf{65.7} & \textbf{68.5} & \textbf{59.0} \\
\midrule
KPConv\,\cite{thomas19ICCV} & \xmark & 65.8 & 93.8 & 98.4 & 82.2 & 0.0 & 20.7 & 55.8 & \textbf{68.9} & 91.3 & 81.9 & 75.3 & 64.9 & 63.5 & 58.8 \\
(Deformable)& \cmark & \textbf{67.2} & \textbf{93.9} & \textbf{98.4} & \textbf{83.5} & 0.0 & \textbf{22.3} & \textbf{60.8} & 66.3 & \textbf{91.7} & \textbf{82.3} & \textbf{76.2} & \textbf{66.7} & \textbf{70.7} & \textbf{60.5} \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-15px}
\caption{\textbf{Semantic segmentation IoU scores on S3DIS Area $\mathbf{5}$.}
We report the mean over 3 trained models.
}
\label{tab:Table_S3DIS_area5} 
\end{table*}


\begin{table*}[t]
\centering
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{rcc|cccccccccccccccccccc}
        \toprule
        Method & \namelong{} & mIoU & wall & floor & cabinet & bed & chair & sofa & table & door & wndw & books. & pic & counter & desk & curtain & fridge & shower & toilet & sink & bathtub & otherf.\\
        \midrule
        MinkNet\,\cite{Choy2019CVPR} & \xmark & 66.7 & 81.0 & 93.8 & 61.0  & \textbf{79.7} & 88.6 & 79.6 & \textbf{71.9} & 55.6 & 57.54 & 75.4 & 25.4 & 55.0 & 61.3 & 61.3 & 44.2 & 61.6 & 85.9 & 61.8 & 79.3 & 53.8 \\
        (5cm) & \cmark & \textbf{69.1} & \textbf{82.1} & \textbf{93.9} & \textbf{63.9} & 79.2 & \textbf{89.2} & \textbf{81.1} & 70.8 & \textbf{59.3} & \textbf{59.8} & \textbf{78.1} & \textbf{25.6} & \textbf{62.2} & \textbf{62.1} & \textbf{67.0} & \textbf{54.1} & \textbf{64.0} & \textbf{89.8} & \textbf{64.1} & \textbf{81.1} & \textbf{54.3}\\
        \midrule
        MinkNet\,\cite{Choy2019CVPR} & \xmark & 72.4 & 85.6 & 96.5 & 64.7 & \textbf{82.1} & 91.0 & 84.4  & 74.5 & \textbf{65.0} & 62.8 & 79.5 & 32.4 & 64.4 & 63.7  & \textbf{75.5} & 51.6  &  \textbf{69.0}  & 93.0  & 67.6 & 87.6  & \textbf{56.3} \\
        (2cm) & \cmark & \textbf{73.6}  & \textbf{86.0}  & \textbf{96.6} & \textbf{66.3} & \textbf{82.1} & \textbf{91.9} & \textbf{86.1} & \textbf{75.7}  & 64.7 & \textbf{64.7} & \textbf{79.6} & \textbf{36.3} & \textbf{67.7} & \textbf{67.0} & 74.7 & \textbf{59.3} & 68.8 & \textbf{93.9} & \textbf{68.6} & \textbf{87.9} & 55.1 \\
        \midrule
        KPConv\,\cite{thomas19ICCV} & \xmark & 68.8 & 82.2 & 94.4 & 63.4 & 77.9 & 88.3 & 76.6 & \textbf{72.8} & 60.0 & 58.4 & 80.1 & 28.6 & 59.3 & 62.7 & 69.9 & 53.1 & \textbf{51.5} & 90.6 & 63.4 & \textbf{86.4} & 55.3 \\
        (Rigid) & \cmark & \textbf{69.5} & \textbf{82.5} & \textbf{94.6} & \textbf{65.3} & \textbf{79.8} & \textbf{89.7} & \textbf{79.0} & 72.2 & \textbf{61.0} & \textbf{58.7} & \textbf{80.1} & \textbf{30.6} & \textbf{60.0} & \textbf{62.8} & \textbf{70.7} & \textbf{55.3} & 50.2 & \textbf{91.5} & \textbf{65.0} & 85.3 & \textbf{55.6} \\
        \midrule
        KPConv\,\cite{thomas19ICCV} & \xmark & 69.3 & 82.4 & \textbf{94.4} & 64.5 & 79.2 & 88.5 & 77.2 & \textbf{73.0} & 60.5 & \textbf{59.1} & \textbf{79.8} & 28.4 & 59.9 & \textbf{63.7} & 71.6 & 53.1 & 54.1 & 91.5 & 63.3 & \textbf{86.0} & \textbf{56.4} \\
        (Deformable) & \cmark & \textbf{70.3} & \textbf{82.6} & \textbf{94.4} & \textbf{65.8} & \textbf{79.5} & \textbf{90.2} & \textbf{79.9} & 72.5 & \textbf{61.7} & 58.2 & 79.6 & \textbf{31.5} & \textbf{62.1} & 63.2 & \textbf{72.0} & \textbf{58.1} & \textbf{56.8} & \textbf{91.8} & \textbf{64.6} & 85.6 & 55.4 \\
        \bottomrule
\end{tabular}
\caption{\small \label{tab:scannet_val_scores} \textbf{Classwise Semantic Segmentation IoU scores on ScanNet validation\,\cite{Dai17CVPR}.}
We report the mean over 3 trained models.
}
\end{table*}


\begin{table*}[t]
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{rcc|cccccccccccccccccccc}
        \toprule
        Method & \namelong{} & mIoU & car & bike & mbike & truck & vehicle & person & cyclist & mcyclist & road & parking & sidewalk & other-gr & building & fence & veget & trunk & terrain & pole & sign \\
        \midrule
        \multirow{2}{*}{MinkNet\,\cite{Choy2019CVPR}} & \xmark & 53.2 & 94.0 & 26.4 & 24.5 & 27.5 & 18.4 & 40.5 & 46.7 & 13.5 & 88.4 & 57.1 & 71.4 & 22.6 & 90.4 & 62.5 & \textbf{83.5} & 65.3 & \textbf{65.8} & 54.0 & 59.1 \\
        & \cmark & \textbf{58.1} & \textbf{95.1} & \textbf{30.6} & \textbf{38.3} & \textbf{43.5} & \textbf{35.3} & \textbf{50.8} & \textbf{51.8} & \textbf{21.9} & \textbf{89.4} & \textbf{59.5} & \textbf{73.0} & \textbf{23.2} & \textbf{90.9} & \textbf{65.2} & 83.3 & \textbf{68.0} & 65.4 & \textbf{57.6} & \textbf{61.7} \\
        \midrule
        \multirow{2}{*}{KPConv\,\cite{thomas19ICCV}} & \xmark & 63.1 & 95.9 & 45.2 & 50.9 & 44.4 & 45.4 & 62.9 & 64.7 & 36.6 & \textbf{89.4} & 65.1 & 73.5 & \textbf{31.3} & \textbf{91.7} & \textbf{67.5} & \textbf{84.4} & 69.4 & \textbf{68.4} & 57.9 & 54.4 \\
        & \cmark & \textbf{63.6} & \textbf{96.4} & \textbf{49.1} & \textbf{59.7} & \textbf{40.5} & \textbf{52.1} & \textbf{69.6} & \textbf{69.3} & \textbf{18.2} & \textbf{89.4} & \textbf{66.2} & \textbf{74.3} & 28.0 & 91.5 & 66.2 & \textbf{84.4} & \textbf{71.0} & 67.9 & \textbf{58.7} & \textbf{54.9} \\
        \bottomrule
\end{tabular}
\caption{\small \label{tab:semkitti_test_results} \textbf{Classwise Semantic Segmentation IoU scores on the SemanticKITTI test set\,\cite{Behley19ICCV}.}}
\end{table*}

